Scalable Multi-Agent Reinforcement Learning through Intelligent Information Aggregation

We consider the problem of multi-agent navigation and collision avoidance when observations are limited to the local neighborhood of each agent. We propose InforMARL, a novel architecture for multi-agent reinforcement learning (MARL) which uses local information intelligently to compute paths for all the agents in a decentralized manner. Specifically, InforMARL aggregates information about the local neighborhood of agents for both the actor and the critic using a graph neural network and can be used in conjunction with any standard MARL algorithm. We show that (1) in training, InforMARL has better sample efficiency and performance than baseline approaches, despite using less information, and (2) in testing, it scales well to environments with arbitrary numbers of agents and obstacles. We illustrate these results using four task environments, including one with predetermined goals for each agent, and one in which the agents collectively try to cover all goals. Code available at https://github.com/nsidn98/InforMARL.

==> icml2023 InforMARL 2/sections/1_introduction.tex <==
\section{Introduction}
Reinforcement Learning (RL) has seen wide-ranging successes recently in high-dimensional robot control \cite{DDPG, RLVisuomotor}, solving physics-based control problems \cite{contControlRL}, playing Go \cite{alphaGo}, Chess \cite{alphaZero} and Atari video games \cite{DQN_Atari, Atari2}, \etc However, challenges remain in many real-world applications in which the tasks cannot be handled by a single agent, e.g., multi-player games, search-and-rescue drone missions, \etc \cite{MARLSurvey}. In such cases, multiple agents may need to work together and share  information in order to accomplish the task \cite{MARLseminal}. Na{\"i}ve extensions of single-agent RL algorithms to multi-agent settings do not work well because of the non-stationarity in the environment, \ie the actions of one agent affect the actions of others \cite{IQL1, IQL2}. Furthermore, tasks may require cooperation among the agents. Classical approaches to optimal planning may (1) be computationally intractable, especially for real-time applications, and (2) be unable to account for complex interactions and shared objectives between multiple agents. The ability of RL to learn by trial-and-error makes it well-suited for problems in which optimization-based methods are not effective. In particular, multi-agent reinforcement learning (MARL) approaches may be suitable in these situations due to their fast run-times and superior performance, and their ability to model shared goals between agents using appropriate reward structures.

%Recent advances in Reinforcement Learning (RL) have led to its success in a wide variety of tasks like high-dimensional robot control \cite{DDPG, RLVisuomotor}, solving physics-based control problems \cite{contControlRL}, playing Go \cite{alphaGo}, Chess \cite{alphaZero} and Atari video games \cite{DQN_Atari, Atari2}, \etc While these results indicate the promise of machine learning, there are cases where the task at hand may be too large for a single agent to handle, as many real-world applications like multi-player games, search-and-rescue drones, \etc, naturally comprise multiple decision makers that interact at the same time \cite{MARLSurvey}. In such cases, multiple agents may work together to exchange knowledge and information from one another in order to accomplish the task \cite{MARLseminal}. Simply extending single-agent RL algorithms to multi-agent settings does not work \cite{IQL1, IQL2} because of the non-stationarity in the environment, \ie, the action of one agent affects the actions of others. Also, some tasks may require cooperation amongst the agents to achieve the objective. Classical approaches for optimal planning may be (a) computationally intractable for real-time applications and (b) unable to model the complex interactions governing the multiple agents and their shared objectives. The natural framework of RL to learn by trial and error and getting rewards as feedback for taking good actions makes it well suited for tasks where optimization-based methods with complex objective functions are not feasible. Thus, multi-agent reinforcement learning (MARL) approaches may be of value for such problems due to their fast run-times, superior performance, and ability to model shared goals using appropriate reward structures.\\

In this paper, we focus on multi-agent navigation and collision avoidance problems in which there are $N$ agents trying to cooperate with each other to collectively solve a task in a 2D environment with static and/or dynamic obstacles. 
% navigating to their respective goals in a 2D environment with static and/or dynamic obstacles. 
% The agents are assumed to be collaborative, \ie  
The rewards are shared across all agents in these collaborative environments. We assume that an agent can only sense the presence of obstacles or other agents within a certain limited radius $r$. 
The overarching objective is for all the agents to complete their tasks in the shortest time possible, while avoiding collisions with other agents and obstacles.
This problem setting is quite general and arises in many contexts, \eg, search-and-rescue robot teams \cite{search_rescue}, environmental monitoring \cite{env_monitoring}, and drone delivery systems \cite{drone_delivery1, drone_delivery2, drone_delivery3}.

MARL-based techniques have achieved significant successes in recent times, \eg, DeepMind's AlphaStar surpassing professional level players in StarCraft II \cite{AlphaStar}, OpenAI Five defeating the world-champion in Dota II \cite{Dota2}, etc. The performance of many of these MARL algorithms depends on the amount of information included in the state given as input to the neural networks \cite{MAPPO}.
% ``\textit{How much information is necessary for multi-agent reinforcement learning agents to learn to perform collision-free navigation in an environment whilst still being scalable?}" 
In many practical multi-agent scenarios, each agent aims to share as little information as possible to accomplish the task at hand. This structure naturally arises in many multi-agent navigation settings, where agents may have a desired end goal but do not want to share their information due to communication constraints or proprietary concerns \cite{satelliteInfoSharing1, satelliteInfoSharing2}. These scenarios result in a decentralized structure, as agents only have locally available information about the overall system's state. In this paper, we focus on the question: ``\textit{Can we train scalable multi-agent reinforcement learning policies that use limited local information about the environment to perform collision-free navigation effectively?}" 
% In this paper, we define decentralized to mean each agent can only sense the positions of the entities in its neighborhood region and is making its own decision according to that local observation.


We propose \textit{InforMARL}, an approach for solving the multi-agent navigation problem using graph-reinforcement learning. The main features of our approach are that it: (1) uses a graph representation of the navigation environment which enables local information-sharing across the edges of the graph; (2) transfers well to different numbers of agents; and (3) achieves better sample complexity in training compared to prior approaches by aggregating relevant local information from neighbors in the underlying graph. More broadly, our work (1) demonstrates that graphs provide a valuable abstraction for multi-agent navigation environments; (2) highlights that more information (\ie global information as states) may not necessarily improve performance, and can, in fact, overwhelm the RL agent networks and lead to increased sample complexity; and (3) shows how graph architectures can identify the most valuable information for navigation from local observations to improve performance and scalability.

%The rest of this paper is organized as follows. In Section \ref{section:related_work}, we briefly summarize recent developments in MARL under different settings. In Section \ref{section:method}, we describe InforMARL, our method for multi-agent navigation in settings with limited observability and communication. In Section \ref{section:experiments}, we show the effectiveness of InforMARL in learning policies for navigation by comparing its performance to other baseline algorithms. We also perform experiments on transferring InforMARL to scenarios with a different number of entities in the environment. Finally, in Section \ref{section:conclusion_future_work}, we discuss the main conclusions of this paper and describe promising directions for future work.


==> icml2023 InforMARL 2/sections/2_related_work.tex <==
\section{Related Work}
% main themes for related work:
% vanilla MARL
% Communication
% Scaling/transferrability
% 
\label{section:related_work}
% In this section, we discuss prior approaches to scaling MARL algorithms, as well as some recent work on information-sharing  between agents in  multi-agent systems.
%An efficient MARL algorithm must be scalable and must account for the non-stationarity of the environment. Improvements to MARL scalability have been studied in several different contexts, with techniques diverging in their inclusion of communications protocols for sharing information amongst agents. In this section, we present recent works that address scaling, communication, and transferability that are most relevant to our work.
Multi-agent navigation problems arise in a number of other contexts, \eg multi-robot navigation. Optimization-based \cite{RVO} and trajectory-based \cite{SIPP,probSafeNav,trajPlan} approaches have been used for multi-robot navigation. However, the former often has long computation times making real-time execution infeasible, while the latter can encounter the ``freezing robot problem" in dense environments due to a large portion of the statespace being marked as unsafe. We therefore focus on MARL approaches. %In this section, we discuss relevant works addressing MARL scaling, communication, and transferability.
\subsection{Scaling MARL}
Research on scaling MARL algorithms has broadly followed two main themes: (1) decentralized execution, and (2) transferring learning between scenarios.

% MARL has been a widely studied topic, especially for different applications like gaming, robotics, etc. A straightforward approach of using independent Q-value functions for each agent using Q-Learning was introduced in \cite{IQL1, IQL2}. This assumes that the other agents are a part of the environment and thus the non-stationarity in the environment results in training instability preventing them from scaling well to more than 2 agents. 
\textbf{Decentralized MARL}:
Centralized-training-decentralized-execution (CTDE) is a popular approach to improve scaling. CTDE frameworks typically use actor-critic methods \cite{ActorCriticSeminal}, where the training step uses a centralized critic that incorporates global information from all actors. During execution, the agents use their own actor networks to select their actions in a decentralized manner. % to improve scalability.  
% CAN WE USE THE NEXT SENTENCE AS A SEGUE TO WHY SINGLE_AGENT RL ALGOS DO NOT WORK?
% A straightforward approach of using independent Q-value functions for each agent using Q-Learning was introduced in \cite{IQL1, IQL2}. This assumes that the other agents are a part of the environment and thus the non-stationarity in the environment results in training instability preventing them from scaling well to more than 2 agents.
% For scaling purposes, researchers have looked into the centralized-training-decentralized-execution (CTDE) framework, which mostly includes utilizing actor-critic methods \cite{ActorCriticSeminal}. The CTDE framework has a centralized critic that incorporates global information from all the actors during training, but in execution, the agents use their own actor networks for selecting actions in a decentralized manner. 
MADDPG \cite{MADDPG} builds upon DDPG \cite{DDPG} by learning a centralized critic that is provided the joint state and actions of all agents. MATD3 \cite{MATD3} uses a double-centralized critic model, reducing the over-estimation bias. \cite{MAPPO} show the effectiveness of PPO in several standard multi-agent environments. VDN \cite{VDN} decomposes a centralized value function to a sum of individual agent-specific functions. Q-Mix \cite{QMIX} improves upon this by imposing a monotonicity requirement on agents' individual value functions and using a learnable mixing of the individual functions.  These MARL algorithms perform well in the navigation environment when they know the positions of all entities in the environment. But, as we will demonstrate, they fail to learn when that information is restricted to just local neighborhoods around the agents.
% While these MARL algorithms perform well in the navigation environment when they have access to the information about the  positions of all entities in the environment, they fail to learn when that information is restricted to just local neighborhoods around the agents. XX TALK ABOUT MOTIVATING EXPERIMENT AS REFERENCE IN A SENTENCE XX.


% KG: currently, this paragraph makes me feel like these approaches will work for our problem -- we need to highlight that these will serve as baselines and our approach will do better than them (explicitly state that they use global info)

% KG: is communication really our main focus? Maybe we want to present limited communication as a feature that enables scaling + transferability?

\textbf{Transferability in MARL}:
It is desirable to have MARL formulations where the number of agents/entities in the environment doesn't hinder the performance of the model. Most of the previous works using MARL for the navigation task require concatenation of observations of other entities in the environment to be able to learn meaningful policies. As the neural network size depends on the state input dimensions used while training, the learned policy fails to work in scenarios with a different number of entities in the environment. With the recent success of graph neural networks, many recent works have focused on leveraging the inherent graph structure present in multi-agent problems and tackling the issue of transferability. Zhou et al. \cite{GNN_IL} create a neighborhood graph according to how close the entities are to each other and use imitation learning to imitate a greedy behavior for the target-coverage problem \cite{targetCoverage1, targetCoverage2}. Similarly, Khan et al. \cite{GPG} use graph neural networks with vanilla policy gradient \cite{policyGradient} for the formation flying task \cite{formationFlying1, formationFlying2}. They show that dynamic graphs have worse performance than static graphs due to the large number of possible graphs the model has to learn. At the beginning of each episode, their model determines the connectivity of the agents with each other and uses the same graph over the whole episode. This works well for the formation flying task as the graph structure does not change much if the agents fly in the same formation over an episode. 
% However, this fails for the navigation task as the graph connectivities can change over time and we show that this approach doesn't work for the navigation scenario. 
DGN \cite{DGN} combines a graph convolutional neural network \cite{GCN} architecture with multi-head attention \cite{AttentionIsAllYouNeed} for a variety of multi-agent environments, including 2D coverage and tracking.
The DGN architecture assumes that each agent communicates with its three closest neighbors. Communicating with the three closest agents leads to a graph that is always connected. However, the three-agent connectivity assumption is highly restrictive in real life applications, as communication is generally restricted by mutual separation due to hardware constraints. Similarly, \cite{G2ANet, GNN_CAV} use an equivalent DGN-like architecture for multi-agent control.
% Further analysis found that distance-based connectivity, as used in \cite{DGN}, leads to the formation of several sub-graphs which cannot communicate with other sub-graphs leading to a significantly harder learning problem. 


We use a distance-based agent-entity graph similar to Entity-Message Passing (EMP) \cite{EMP}. However, the EMP architecture assumes that the agents have access to the positions of all entities in the environment at the beginning of the episode, which is not possible if there are occluded static or dynamic obstacles.
% A major assumption in their work is that the agents have access to the positions of all the entities at the beginning of the episode. From a practical standpoint this works well in scenarios which only have static obstacles with their positions already known but fails in scenarios where there are unknown static or dynamic obstacles. 
By contrast, our model does not make this assumption.
% Our graph construction approach is also distance-based and is closely related to \cite{EMP}. However, \cite{EMP} assumes that the agents have access to the positions of all the entities at the beginning of the episode, which is not possible in the navigation setting where there are occluded static or dynamic obstacles.

% DGN (Jiang et al., 2018) also uses a similar mechanism for communication but with Q-learning (Mnih et al., 2013) for training. They allowed each agent to communicate with its 3 closest neighbors. From a practical consideration, communication between agents is usually restricted by their mutual separation, meaning that an agent can communicate only with neighbors within a certain radius. We would also like to emphasize that being able to communicate with the 3 closest neighbors ensures that the agents’ graph is always a single connected component and no agents are ever disconnected from the others, while having a distance-based restriction leads to formation of several different connected components in the agents’ graph, none of which can communicate with each other leading to a significantly more difficult learning (to cooperate) problem.

\subsection{Information Sharing for MARL}
For various cooperative tasks where explicit coordination is required to solve the task, enabling communication to share information across the agents helps with the performance.
In CommNet \cite{CommNet}, the authors introduce a model to learn a differentiable communication protocol between multiple agents. However, it does not explicitly model the interactions between the agents but rather averages the states of all the neighboring agents. VAIN \cite{VAIN} improves upon CommNet by using an exponential kernel-based attention to choose specific messages from other agents to attend to. Similarly, ATOC \cite{ATOC} and TarMAC \cite{TarMAC} use an attention mechanism for communication among agents but without any restrictions on which agent can communicate with which others, leading to centralization during execution. 
% Just adding all related work stuff after this for reference, we can prune and word it better so that it flows well with context.
GAXNET \cite{GAXNet} also uses an attention mechanism \cite{AttentionIsAllYouNeed}, but additionally allows for the exchanging of weights with other agents to reduce the attention mismatch between them. While their model is shown to work well for navigation, it requires the maximum number of agents in the environment to be fixed before training. We also use an attention mechanism for inter-agent communication. However, we do not have any message passing between objects in the environment (also called 'entities') and agents; instead, the agents themselves do all the computation with local information of the entities’ states.
% they replace with zero if unobservable which fits in the POMDP setting but still need a fixed vector hence the max number of agents is fixed at the beginning.
% MAGIC

% Karthik's attempt at restructuring this section
% \begin{comment}

% Developing a scalable MARL framework has been studied by several researchers and a popular approach is the  centralised-training-decentralised-execution (CTDE) framework. The CTDE framework  typically utilizes actor-critic methods \cite{ActorCriticSeminal}, and uses a centralised critic which gets global information from all the actors during training, but while execution, the agents just use their actor networks in a decentralised manner to improve scalability. One approach is MADDPG \cite{MADDPG}, which builds upon DDPG \cite{DDPG} by learning a centralised critic using the joint state and actions of all agents. MATD3 \cite{MATD3} uses a double-centralised critic model which helps in reducing the over-estimation bias. The CTDE framework has also been applied to value-based methods, as in shown in \cite{VDN}. 
% % some version of this is needed in the end of the scalability references to state why they dont work right off the bat for us or why they are different than our work
% While these frameworks help in scaling, we show that their success on the multi-agent navigation problem is limited because of XYZ, and our work improves these methods for the MANP. 

% % about transferability
% Prior works that use MARL for navigation tasks require a concatenation of observations from all agents to be learn meaningful policies \cite{XXX}. However, since the neural network size depends on the state input dimensions used while training, the learnt policy fails to generalise well to scenarios with a different number of agents. Recently, many works have focused on leveraging the inherent graph structure present in multi-agent problems and tackle the issue of transferability \cite{GNN_IL, targetCoverage1, targetCoverage2}.
% Khan et al. \cite{GPG} use graph neural networks with vanilla policy gradient \cite{policyGradient} for the formation flying task.
% % However, their approach works well only when the graph structure does not change too much, as in the case of formation flying, and fails for navigation problems where the graphs are dynamic. 
% DGN \cite{DGN} combines a graph convolutional neural network \cite{GCN} architecture with multi-head attention \cite{AttentionIsAllYouNeed} for a variety of multiagent environments, including 2D navigation. The DGN architecture assumes that each agent communicates with three of its closest neighbours, which may not be possible in real-world navigation problems with obstacles and hardware constraints. Furthermore, distance-based connectivity for navigation tasks often leads to the formation non-communicating sub-graphs making the learning significantly harder. Our graph construction approach is also distance-based and is closely related to \cite{EMP}. However, \cite{EMP} assumes that the agents have access to the positions of all the entities at the beginning of the episode, which is not possible in the navigation setting where there are occluded static or dynamic obstacles.

% % A major assumption in their work is that the agents have access to the positions of all the entities at the beginning of the episode. From a practical standpoint this works well in scenarios which only have static obstacles with their positions already known but fails in scenarios where there are unknown static or dynamic obstacles. In contrast, our model doesn't require the positions of all the entities at the beginning of the episode. 

% % In contrast, our model doesn't require the positions of all the entities at the beginning of the episode. --> Not clear what it means!



% \end{comment}

==> icml2023 InforMARL 2/sections/3_methodology.tex <==
% (refer to the figure and explain each module)
% Environment module:
    % Explain construction of graphs  (done)
    % Explain POMDP (done)
    % Explain local, nbd, global state space (done_
    % Explain reward structure (done)
% Information Aggregation module:
    % Explain the concatenation of graph message + local state (done)
    % Explain the entity encoding layer + graph transformer
% Action selection module:
    % Just say that we are using MAPPO as the base RL algo with actor and value networks with RNN as the base layers (done)

    \begin{figure*}[t!]
        \centering
        \includegraphics[width=0.92\textwidth]{figures/graphMARLArch.v8.png}
        \caption{Overview of InforMARL. (i) Environment: The agents are depicted by green circles, the goals are depicted by red rectangles, and the unknown obstacles are depicted by gray circles. $x^{(i)}_{agg}$ represents the aggregated information from the neighborhood, which is the output of the GNN. A graph is created by connecting entities within the sensing-radius of the agents. (ii)  Information Aggregation: Each agent's observation is concatenated with $x^{(i)}_{\mathrm{agg}}$. The inter-agent edges are bidirectional, while the edges between agents and non-agent entities are unidirectional. (iii) Graph Information Aggregation: The aggregated vector from all the agents is averaged to get $X_{\mathrm{agg}}$.
        (iv) Actor-Critic: The concatenated vector $[o^{(i)}, x^{(i)}_{\mathrm{agg}}]$ is fed into the actor network to get the action, and $X_{\mathrm{agg}}$ is fed into the critic network to get the state-action values.}
        \label{fig:arch}
    \end{figure*}
    
\section{Description of InforMARL}
    \label{section:method}
    Our MARL framework for navigation, InforMARL, consists of four modules, as shown in Figure \ref{fig:arch} and described below. 
    \subsection{Environment}
        \label{section:env}
        Every object in the environment (also known as an `entity') is assumed to be either an agent, an obstacle, or a goal/landmark. We define an agent-entity graph with respect to agent $i$ at each time-step $t$, as $g^{(i)}_t \in \mathcal{G}: (\mathcal{V}, \mathcal{E})$, where each node $v\in\mathcal{V}$ is an entity in the environment. The variable \texttt{entity\_type(j)}$\in\{ \texttt{agent}, \texttt{obstacle}, \texttt{goal}\}$ determines the type of entity at node $j$. 
        There exists an edge $e\in\mathcal{E}$ between an agent and an entity if they are within a `sensing radius' $\rho$ of each other. The agent-agent edges are bidirectional, whereas the agent-non-agent edges are unidirectional (\ie messages can only be passed from the non-agent entity to the agent). In other words, a unidirectional edge is equivalent to the agent sensing a nearby entity's state, while a bidirectional edge is equivalent to a communication channel  between agents. This structure is similar to the agent-entity graph defined in \cite{EMP}, but without the assumption that all agents have access to the positions of all entities at the beginning of each episode. Note that our formulation also supports cases where disconnected sub-graphs are formed due to the positioning of the entities in the environment. 

        The corresponding Decentralized Partially Observable Markov Decision Process (Dec-POMDP) \cite{MDP, POMDP1, POMDP2} is characterized by the tuple $\langle N, S, O, \mathcal{A}, \mathcal{G}, P, R,\gamma \rangle$, where $N$ is the number of agents, $s\in S = \mathbb{R}^{N\times D}$ is the state space of the environment and $D$ is the dimension of the state, and $o^{(i)}=O(s^{(i)})\in \mathbb{R}^{d}$ is the local observation for agent $i$, where $d\leq D$ is the observation dimension. 
        $a^{(i)} \in \mathcal{A}$ is the action space for agent $i$ and the joint action for all $N$ agents is given by $A=(a^{(1)},\cdots,a^{(N)})$. %Specifically, $a^{(i)}\in  \mathbbm{1}^{|\mathcal{A}|}$ where $a^{(i)}$ is a one-hot vector of size equal to the number of possible actions. 
        Specifically, $a^{(i)}$ is a one-hot vector of size equal to the number of possible actions. $g^{(i)} \in \mathcal{G}(s; i)$ is the graph network formed by the entities in the environment with respect to agent $i$. $P(s'|s, A)$ is the transition probability from $s$ to $s'$ given the joint action $A$. $R(s, A)$ is the joint reward function. $\gamma \in [0,1)$ is the discount factor. The MARL training process seeks to find an optimal policy, $\Pi= \left(\pi^{(1)}, \cdots, \pi^{(N)}\right)$, where each agent uses a policy $\pi_\theta^{(i)}\left(a^{(i)}|o^{(i)}, g^{(i)}\right)$ parameterized by $\theta$ to determine its action $a^{(i)}$ from its local observation $o^{(i)}$ and the graph network $g^{(i)}$ that it is a part of, while optimizing the discounted accumulated reward $J(\theta) = \mathbb{E}_{A_t, s_t}\left[\sum\limits_t \gamma^t R\left(s_t, A_t\right)\right]$.
    
        Agent $i$'s local observation $o^{(i)}$ consists of its position and velocity in a global frame of reference and the relative position of the agent's goal with respect to its position.
        Each node $j$ on the graph $g^{(i)}$ has node features $x_j=[p^j_i, v^j_i, p^{\mathrm{goal},j}_i, \texttt{entity\_type(j)}]$ where $p^j_i, v^j_i, p^{\mathrm{goal},j}_i$ are the \emph{relative} position, velocity, and position of the goal of the entity at node $j$ with respect to agent $i$, respectively. If node $j$ corresponds to a (static/dynamic) obstacle or a goal, we set $p^{\mathrm{goal},j}_i \equiv p^j_i$. 
        % This is because inferring the goal/intent of other entities by using just sensors is impossible.
         Each edge $e_{ij}$ has an associated edge feature given by the Euclidean distance between the entities $i$ and $j$. For processing the \texttt{entity\_type} categorical variable, we experimented with both using an embedding layer \cite{word2vec} and using one-hot encoding. No significant performance advantage with one method over the other was found, so we chose to use the embedding layer. Further analysis revealed that the learned embedding vectors for \texttt{entity\_type} were equidistant from each other when visualized in 2D. This was to be expected because each of the entity types $(agent, obstacle, goal)$ are equally distinct from another. Future work could include further refinement of \texttt{entity\_type}, \eg, adversarial vs. cooperative obstacles, static vs. dynamic obstacles, etc.

We adopt a similar reward function as used in multi-agent particle environment (MAPE) %\footnote{\href{https://github.com/openai/multiagent-particle-envs}{https://github.com/openai/multiagent-particle-envs}} 
 \cite{MAPE} where the joint reward function is defined as $R(s_t,A_t)=\sum_{i=1}^{N}r_t^{(i)}$, which encourages cooperation among all agents. Here $r_t^{(i)}$ is each agent's reward at timestep $t$ and depends on the scenario. Details about the reward functions for the different task environments can be found in Appendix \ref{appendix:env}.
 % where each agent $i$ gets a reward: $r_t^{(i)} = r_{\mathrm{dist},t}^{(i)} + r_{\mathrm{coll},t}^{(i)} + r_{\mathrm{goal},t}^{(i)}$, where $r_{\mathrm{dist}, t}^{(i)}$ is the negative of the Euclidean distance to the goal, $r_{\mathrm{coll},t}^{(i)}=-5$ if it collides with any other entity and zero otherwise, and $r_{\mathrm{goal},t}^{(i)}=+5$ if the agent has reached the goal and zero otherwise. The joint reward function is defined as $R(s_t,A_t)=\sum_{i=1}^{N}r_t^{(i)}$, which encourages cooperation among all agents.

\subsection{Information Aggregation}
    \label{section:info_agg}
    To infer information about the local neighborhood around each agent $i$, we use a graph neural network (GNN) with a message passing framework \cite{message_passing_GNN}. Specifically, we use Unified Message Passing Model (UniMP) \cite{graphTransformerConv}, a variant of a graph transformer \cite{AttentionIsAllYouNeed, graphTransformer} where each layer update is defined as $x_i' = W_1 \cdot x_i + \sum\limits_{j\in\mathcal{N}(i)}\alpha_{i,j}W_2 \cdot x_j$, %follows:
    % \begin{equation}
    %     x_i' = W_1 \cdot x_i + \sum\limits_{j\in\mathcal{N}(i)}\alpha_{i,j}W_2 \cdot x_j,
    % \end{equation}
    where $x_k$ are the node features in the graph, $\mathcal{N}(i)$ is the set of nodes which are connected to node $i$, $W_k$ are learnable weight matrices and the attention coefficients $\alpha_{i,j}$ are computed via multi-head dot product attention:
    \begin{equation}
        \alpha_{i,j} = \mathrm{softmax}\left(\dfrac{\left(W_3 \cdot x_i\right)^T\left(W_4 \cdot x_j + W_5 \cdot e_{ij}\right)}{\sqrt{\mathrm{c}}}\right)
    \end{equation}
    where %$W_k$ are learnable weight matrices, 
    $e_{ij}$ are edge features for the edge connecting nodes $i$ and $j$, and $c$ is the output dimension for that specific layer.
    
    The attention mechanism allows the agents to selectively prioritize messages coming from their neighbors according to their importance. We use multiple layers of this message-passing so that information can be propagated between agents that are higher-order neighbors with each other. For each agent $i$, this module aggregates information from the neighboring nodes in the graph into a fixed-sized vector $x^{(i)}_{\mathrm{agg}}$. The concatenated vector $[o^{(i)}, x^{(i)}_{\mathrm{agg}}]$ is given as the input to the actor network. This architecture allows InforMARL to dynamically adapt to a changing number of entities in the environment while remaining invariant to the permutation of the observed entities.

\subsection{Graph Information Aggregation}
    \label{section:graph_info_agg}
    While training a model in the CTDE setting, the critic generally gets the state-action pairs of all individual agents in the environment as a concatenated vector. To make the training transferable to a variable number of agents and to aid with curriculum learning \cite{curriculum_learning, transfer_learning1, transfer_learning2}, we replace this concatenation with a graph information aggregation module. This module is similar to the `Information Aggregation' one in which a GNN aggregates information from the agent's neighbors. A global mean pooling operator,  $X_{\mathrm{agg}} = \frac{1}{N}\sum\limits_{i=1}^N x^{(i)}_{\mathrm{agg}}$, is applied to aggregate the updated node features in the graph. %:
    % \begin{equation}
    %     X_{\mathrm{agg}} = \frac{1}{N}\sum\limits_{i=1}^N x^{(i)}_{\mathrm{agg}}
    % \end{equation}
    Note that $X_{\mathrm{agg}}$ is a vector of fixed size independent of the number of agents, which is not the case when concatenating the state action-pairs of all individual agents. This vector is then given as input to the critic network.

\subsection{Actor-Critic Networks}
    \label{section:actor_critic}
    The actor and critic networks can be either a multi-layer perceptron (MLP) or a recurrent neural network (RNN) \cite{rnnForPOMDP}, using either LSTMs \cite{LSTM} or GRUs \cite{GRU}. Our proposed information aggregation method can be used in conjunction with any standard MARL algorithm (\eg, MADDPG \cite{MADDPG}, MATD3 \cite{MATD3}, MAPPO \cite{MAPPO}, QMIX \cite{QMIX}, VDN \cite{VDN}, etc.). 




==> icml2023 InforMARL 2/sections/4_experiments.tex <==
\section{Experiments}
\label{section:experiments}
% Explain the modifications made to MAPE to get our navigation env
% Brief overview of baseline algorithms and the modifications made to port to our navigation environment

% Experiments to include:
% 1: Local-nbd-global for mappo and explain the importance of information (DONE)
% 2: 3-agents learning curves for 
    % Global or Local MARL (DONE)
    % GPG (DONE)
    % EMP (TODO)
    % DGN + ATOC (DONE)
    % Ours (DONE)
% 3: Ablation radius for graph connectivity (DONE)
% 4: Ablation for cent_obs vs no cent_obs (DONE)
% 5: 7,10-agents learning curves for same algos as above (TODO)

% Transfer Learning from 3-5 (TODO)

% Many of the baselines will not have good performance in our environment and we can exclude them for experiments with more agents.
% Give possible reasons for why a particular baseline doesn't work in our environment (we have valid reasons for 
    % GPG: static graphs + entity info not included, 
    % DGN + ATOC: entity info not included in graph
    % EMP: Assumption of knowing the position of all entities at the beginning of the episode hampers performance.
    % Local MARL: Entity information not included, 
    % Nbd-MARL: Not sufficient information and network size becomes bigger when more nbd entities considered)
    % Also, make a note that all the baseline implementations were modified from their authors' original codebase.
    
% Get metrics (reward over episode while testing, num_collisions)
% Run experiments with transferring to a different environment compared to what it was trained on (eg: train-on-3 and test-on-7)
% Run experiments with curriculum learning

% \subsection{Task Description}
\textbf{Environment descriptions}: We evaluate our proposed model on four different navigation tasks by modifying the MAPE \cite{MAPE}. In all these environments, $N$ agents move around in a 2D space following a double integrator dynamics model \cite{double_integrator_model}. Each agent has a discrete action space where it can control unit acceleration and deceleration in the $x$- and $y$- directions. 
% Agents are rewarded based on how far any agent is from each landmark. Agents are penalized if they collide with other agents. So, agents have to learn to cover all the landmarks while avoiding collisions.
% The  objective is for the agents to deploy themselves in a manner such that every agent reaches a distinct
% landmark. Note that we do not assign particular landmark to each agent, but instead let the agents
% communicate with each other and develop a consensus as to who goes where.
% \begin{CompactItemize}
%     \item \textbf{Coverage} \cite{targetCoverage1, targetCoverage2}: Each agent is supposed to cover a distinct landmark/goal while avoiding collisions with other entities in the environment.
%     \item \textbf{Target (SUGGEST A NAME FOR THIS)}: The target task differs from the coverage task in that each agent navigates to its own specific goal rather than any of the available goals. Static obstacles are placed randomly in the environment in each episode. 
%     % Agents start at random locations at the beginning of each episode; the corresponding goals are also randomly distributed. 
% % The overarching objective is for every agent to reach its corresponding goal without colliding with any other entity. 
%     \item \textbf{Formation} \cite{EMP}: There are $N$ agents and 1 landmark in the environment. The agents have to position themselves in an $N$-sided regular polygon with the landmark at its centre.
%     \item \textbf{Line} \cite{EMP}: There are $N$ agents and 2 landmarks in the environment and the agents have to position themselves equally spread out in a line between the two landmarks.
% \end{CompactItemize}
\begin{CompactEnumerate}
%    \itemsep0em 
    \item \textbf{Target}: 
    Each agent tries to reach its preassigned goal while avoiding collisions with other entities in the environment.
    %The target task differs from the coverage task in that each agent navigates to its own specific goal rather than any of the available goals. Static obstacles are placed randomly in the environment in each episode. 
    \item \textbf{Coverage} \cite{targetCoverage1, targetCoverage2}: Each agent tries to go to a goal while avoiding collisions with other entities, and ensuring that no more than one agent reaches the same goal.
    % Each agent is supposed to cover a distinct landmark/goal while avoiding collisions with other entities in the environment.
    % Agents start at random locations at the beginning of each episode; the corresponding goals are also randomly distributed. 
% The overarching objective is for every agent to reach its corresponding goal without colliding with any other entity. 
    \item \textbf{Formation} \cite{EMP}: There is a single landmark (the counterpart of a goal for this task), and the agents try to position themselves in an $N$-sided regular polygon with the landmark at its centre.
    \item \textbf{Line} \cite{EMP}: There are two landmarks, and the agents try to position themselves equally spread out in a line between the two.
\end{CompactEnumerate}
We first focus on the \emph{Target} task environment in this section, and present the performance of InforMARL on the other tasks in Section \ref{sec:other_tasks}. More details about the environments can be found in Appendix \ref{appendix:env}.


% \subsection{Implementation Specifications}
\noindent \textbf{Implementation specifications}:
    We chose to use MAPPO \cite{MAPPO} as the base MARL algorithm for InforMARL because it was found to be the best performing of the standard MARL baselines in the 3 agent-3 obstacle \emph{Target} environment. We implemented InforMARL by modifying the official codebase for MAPPO in PyTorch. The codebase links to our baseline implementations can be found in Appendix \ref{appendix:implementation}. %\ref{appendix:implementation}. 
    We used the official implementations for most of the baselines considered in Section \ref{sec:comparison_algos}. We prefix the algorithm name with `R' to denote the recurrent neural network (RNN) version of the algorithm (\eg MAPPO-RMAPPO, \etc).
    We use the same hyperparameters as used in the experiments for MAPPO, and do not perform parameter tuning on InforMARL for any of the MAPPO-based parameters. The hyperparameters used in our experiments can be found in Appendix \ref{appendix:hyperparams}.
    % We train the models with five different random seeds, and compute the means and standard deviations of the rewards. %in Figures \ref{fig:compare_plots}, \ref{fig:compare_rad}, and \ref{fig:cent_obs}.

\noindent \textbf{Amount of information available to agents}: The amount of information available to each agent determines whether or not it can learn a meaningful policy. Although having more information generally translates to better performance, it does not necessarily scale well with the number of agents. Prior works \cite{MAPPO, MADDPG} have typically used a na{\"i}ve concatenation of the states of all agents or entities in the environment fed into a neural network. Such an approach scales poorly (the network input size is determined by the number of agents) and does not transfer well to scenarios with a different number of agents than the training environment. We vary the amount of information available to agents by defining three information modes: 
%had global information about the environment fed into the neural networks by na{\"i}vely concatenating the states of individual entities in the environment. 
%The network input size is determined by the number of agents in the environment and doesn't allow for transferability to different scenarios from those it was trained on. To show the variation in the learned policies with the amount of information available in the observations of the individual agents, we define three different information modes for the baseline MARL methods:
    \begin{itemize}
        \itemsep0em 
        \item \emph{Local:} In the local information mode, $o^{(i)}_{\mathrm{loc}} = [p^{(i)}, v^{(i)}, p^{(i)}_{\mathrm{goal}}]$ where $p^{(i)}$ and $v^{(i)}$ are the position and velocity of agent $i$ in a global frame, and $p^{(i)}_{\mathrm{goal}}$ is the position of the goal relative to the agent's position. InforMARL uses this information mode.
        \item \emph{Global:} Here, $o_{\mathrm{glob}}^{(i)} = [p^{(i)}, v^{(i)}, p^{(i)}_{\mathrm{goal}}, p^{(i)}_{\mathrm{other}}]$, where $p^{(i)}_{\mathrm{other}}$ comprises of the relative positions of all the other entities in the environment. The scenarios defined in the MAPE (and consequently, other approaches that use MAPE) use this type of information mode unless explicitly stated otherwise.
        \item \emph{Neighborhood:} Here, agent $i$ observes $o_{\mathrm{nbd}}^{(i)} = [p^{(i)}, v^{(i)}, p^{(i)}_{\mathrm{goal}}, p^{(i)}_{\mathrm{other}}]$, where $p^{(i)}_{\mathrm{other}}$ comprises of the relative positions of all other entities which are within a distance \texttt{nbd-dist} of the agent. The maximum number of entities within the neighborhood is denoted \texttt{max-nbd-entities}, and so the dimension of the observation vector is fixed. If there are fewer than \texttt{max-nbd-entities} within a distance \texttt{nbd-dist} of the agent, we pad this vector with zeros.
    \end{itemize}
    % \begin{CompactItemize}
    %     \item \emph{Local:} In the local information mode, $o^{(i)}_{\mathrm{loc}} = [p^{(i)}, v^{(i)}, p^{(i)}_{\mathrm{goal}}]$ where $p^{(i)}$ and $v^{(i)}$ are the position and velocity of agent $i$ in a global frame, and $p^{(i)}_{\mathrm{goal}}$ is the position of the goal relative to the agent's position. InforMARL uses this information mode.
    %     \item \emph{Global:} Here, $o_{\mathrm{glob}}^{(i)} = [p^{(i)}, v^{(i)}, p^{(i)}_{\mathrm{goal}}, p^{(i)}_{\mathrm{other}}]$, where $p^{(i)}_{\mathrm{other}}$ comprises of the relative positions of all the other entities in the environment. The scenarios defined in the MAPE (and consequently, other approaches that use MAPE) use this type of information mode unless explicitly stated otherwise.
    %     \item \emph{Neighborhood:} Here, agent $i$ observes $o_{\mathrm{nbd}}^{(i)} = [p^{(i)}, v^{(i)}, p^{(i)}_{\mathrm{goal}}, p^{(i)}_{\mathrm{other}}]$, where $p^{(i)}_{\mathrm{other}}$ comprises of the relative positions of all other entities which are within a distance \texttt{nbd-dist} of the agent. The maximum number of entities within the neighborhood is denoted \texttt{max-nbd-entities}, and so the dimension of the observation vector is fixed. If there are fewer than \texttt{max-nbd-entities} within a distance \texttt{nbd-dist} of the agent, we pad this vector with zeros.
    % \end{CompactItemize}
    
\subsection{A Motivating Experiment \label{sec:motivating_expt}}
    The \emph{local} or \emph{neighborhood} information modes are transferable to scenarios with a different number of entities in the environment. By contrast, the \emph{global} information mode is not transferable to other scenarios. Figure \ref{fig:local_nbd_global} shows the rewards obtained during training using the three information modes in the \emph{Target} task environment. 
    % We use RMAPPO as the base MARL algorithm for the 3 agent-3 obstacle scenario. We chose RMAPPO because it was found to be the best-performing MARL algorithm in the global information mode. 
    
    \begin{figure}[h!]
        \centering
        % \includegraphics[width=\linewidth]{plots/local_nbd_global.png}
        \includegraphics[width=0.8\linewidth]{plots/local_nbd_global.pdf}
         \setlength{\belowcaptionskip}{-12pt}
        \caption{RMAPPO with the local, neighborhood (with 1, 3, and 5 \texttt{max-nbd-entities}), and global information given as states. The plots show the rewards during training for the 3 agent-3 obstacle \emph{Target} task environment. 
        % The means and standard deviations of the rewards over training with five random seeds are shown. 
        Comparing the global information mode to the others, we see that merely providing local information and a na{\"i}ve concatenation of neighborhood information is not sufficient to learn an optimal policy.}
        \label{fig:local_nbd_global}
    \end{figure}
    
   We see in Figure \ref{fig:local_nbd_global}  that the policy learned with global information is better than the policies learned with local or neighborhood information. This is because it has the information necessary to take optimal actions. In the `nbd\_5' scenario, if all entities are within the \texttt{nbd\_dist} ball, then $o^{(i)}_{\mathrm{nbd}}\equiv o^{(i)}_{\mathrm{glob}}$, since there are only five entities in the environment apart from the agent itself.
    Although the `nbd\_5' scenario is almost similar to the global information mode, the performances are not similar: the global information mode achieves much higher rewards. This behavior is because the observation $o_{i,\mathrm{nbd}}$ can change temporally from having information about an entity when it lies within a \texttt{nbd\_dist} ball of the agent, and then getting padded with zeros when it is out of the ball. This inconsistency in the amount of information accessible to the agent at every time step causes a significant performance difference between the policies learned with global and neighborhood information modes. This experiment motivates us to find a way in which more information can be leveraged (similar to the global case), but in a manner that does not suffer from the performance shortcomings of the neighborhood or local information modes. 


\subsection{Comparison of InforMARL with Other Baselines} \label{sec:comparison_algos}
 \begin{figure*}[h!]
%        \centering
%        \begin{subfigure}[b]{0.75\columnwidth}
\includegraphics[width=0.33\textwidth]{plots/compare_3_short.pdf}
            % \caption{3 agents}
 %           \label{fig:compare_3}
 %       \end{subfigure}%
  %      
  %      \begin{subfigure}{0.75\columnwidth}
            %\centering      
            \includegraphics[width=0.33\textwidth]{plots/compare_7_short.pdf}
            % \caption{7 agents}
%            \label{fig:compare_7}
 %       \end{subfigure}
 %       
 %       \begin{subfigure}{0.75\columnwidth}
  %          \centering         
  \includegraphics[width=0.33\textwidth]{plots/compare_10_short.pdf}
            % \caption{10 agents [THIS IS NOT FINAL]}
%            \label{fig:compare_10}
 %       \end{subfigure}
 %       
 %       \begin{subfigure}{0.75\columnwidth}
      \centering   \includegraphics[width=0.8\textwidth]{plots/legend_3_short_transpose.png}
            % \caption{legend}
%            \label{fig:legend}
%        \end{subfigure}
%\vspace{-0.1in}
        \caption{Comparison of the training performance of InforMARL with the best-performing baselines using global and local information in the \emph{Target} task environment. The means and standard deviations of the rewards over training with five random seeds are shown. InforMARL significantly outperforms most baseline algorithms. Although RMAPPO has similar performance, it requires global information. Appendix \ref{appendix:full_comparison} presents a complete comparison to more baselines.}
        % \ref{appendix:full_comparison}.}
        \label{fig:compare_plots}
    \end{figure*}
    
    As shown in Section \ref{sec:motivating_expt}, using local information modes or na{\"i}vely concatenating neighborhood entity information is not sufficient to learn optimal policies. In this section, we demonstrate that InforMARL can effectively learn policies for navigation given local information. We then compare its performance  in the \emph{Target} environment with prior deep MARL approaches. Specifically, we consider the following methods as baselines for comparison.
    % ADD ONE LINE SUMMARY ABOUT ALL THESE ALGOS
    \begin{CompactEnumerate}
   \item \textbf{Graph Policy Gradient (GPG) \cite{GPG}:} GPG uses a graph convolutional neural network (GCN) \cite{GCN} to parameterize policies for agents. The authors use the policy gradient method \cite{policyGradient} as the base MARL algorithm. We perform experiments with both dynamic and static graphs. \textit{(Note: It was shown in \cite{GPG} that using a static graph constructed at the beginning of the episode was better than using a dynamic graph.)}
    \item \textbf{Graph Convolutional Reinforcement Learning (DGN, DGN+ATOC) \cite{ATOC, DGN}:} Similar to GPG, these methods use GCNs to capture interactions between the agents in the environment. A key difference between InforMARL and these two methods (GPG and DGN) is that while the latter two approaches consider only agents in their message-passing graph, InforMARL also includes other (non-agent) entities in the graph.
    \item \textbf{Entity Message Passing (EMP) \cite{EMP}:} Similar to InforMARL, EMP uses an agent-entity graph. However, in contrast to InforMARL, EMP assumes that agents know the positions of all entities in the graphs (i.e., global information) at the beginning of the episode. 
    \item \textbf{Other standard MARL Algorithms:} Finally, we compare InforMARL with standard MARL algorithms, namely, MADDPG \cite{MADDPG}, MATD3 \cite{MATD3}, QMIX \cite{QMIX}, VDN \cite{VDN} and MAPPO \cite{MAPPO}. In each case, we also consider the recurrent neural network versions. We focus on results for the global information modes, we found that these methods did not learn well with just local information.
    \end{CompactEnumerate}
    
    % discussion of comparison plots
    Figure \ref{fig:compare_plots} shows the training performance of InforMARL and the  best-performing of the baselines mentioned above for the \emph{target} task environment. For ease of visualization, we plot only the four best-performing methods with global and local information, respectively. Each line corresponds to the mean and standard deviation over five random seeds.  We consider scenarios with $N = \{3, 7, 10\}$ agents. Comparisons to other baselines can be found in Appendix \ref{appendix:full_comparison}, and ablation studies for varying sensing radii in Appendix \ref{appendix:ablation}.
    
   Figure \ref{fig:compare_plots} illustrates that only using RMAPPO (\ie the RNN version of MAPPO) or InforMARL, agents are able to learn to navigate and get to their goals. However, unlike RMAPPO which requires global information, InforMARL achieves this with just local information. Furthermore, InforMARL requires a similar number of training steps as RMAPPO, despite having access to much less information.    
    
    \begin{table*}\small
        \begin{tabular}{|c||p{0.3in}||c|c|r|c||c|c|r|c||c|c|r|c|}
        % \specialrule{.2em}{.0em}{0em} 
        \hline
        \multirow{2}{*}{\bf Algorithm} & {\bf Info} & \multicolumn{4}{c||}{$\boldsymbol{N=3}$} & \multicolumn{4}{c||}{$\boldsymbol{N=7}$} & \multicolumn{4}{c|}{$\boldsymbol{N=10}$}\\
        % \specialrule{.2em}{.0em}{0em} 
        \cline{3-14}
         & {\bf mode} & Reward & $T$ & \# col  & $S\%$ & Reward & $T$ & \# col & $S\%$ & Reward & $T$ & \# col & $S\%$\\
    % &mode & & &  & & & &  & & & &  & \\ 
    \hline \hline
    % \specialrule{.2em}{.0em}{0em} 
    % & & Reward & T & \# Collisions & Reward & T & \# Collisions & Reward & T & \# Collisions \\ \hline
    % [ 9.26742051, 14.89032852,  3.50379812, 11.14161186, 25.31587059,
    %   17.04159552, 12.54459496, 10.00575196,  9.44997091,  4.68431054,
    %     8.62389318,  4.06287585,  9.22936928, 13.21598668, 10.50795341])
        % MADDPG           & Global          &   $-100.73$     & $0.97$  &      $1.60$   &   5   &   $-206.07$     &  $0.98$ &    $6.01$      &   0  &  -210.43   &  1.00 &   9.26    &   0     \\ \hline
        RMADDPG          & Global          &   $10.73$     &  $0.75$ &         $1.72$   &  23 & $-122.07$  & $0.95$  & $4.61$ &  3 &     -127.98          &  1.00      &  7.39 &      0         \\ \hline
        % MATD3             & Global          &   $-90.31$     &  $0.98$ &    $1.11$     & 5 &   $-169.08$     & $0.99$  &         $1.98$      & 1  &  -173.20   &  1.00 &   3.50 &    0       \\ \hline
        RMATD3           & Global          &   $105.49$     & $0.51$  &     $1.62$      &  67  &     $-128.93$   & $0.96$  &      $3.67$         &  6  &  -131.72  & 0.99   &  5.94  &    1       \\ \hline
        % QMIX              & Global          &   $-54.24$     &  $0.84$ &         $2.06$      & 7  &  $-288.81$   & $0.97$  &     $17.05$     &  0    &     -273.46   & 1.00  & 25.31 &       0      \\ \hline
        RQMIX           & Global          &    $19.21$    &  $0.77$ &       $0.83$     & 28  &   $-83.41$     & $0.85$  &    $5.83$      & 12 &   -76.98     &  0.96 &  8.65  &     2      \\ \hline
        % VDN              & Global          &   $18.86$     &  $0.67$ &        $2.29$       & 27 &  $39.87$    & $0.64$  &      $8.58$   &  23  &    43.23    &  0.73 &  12.54  &    19       \\ \hline
        RVDN             & Global          &    $64.04$    &  $0.62$ &          $0.57$     &  45  &  $140.94$  &  $0.62$ &       $3.42$   &   47  &    157.63    &  0.64 &  4.93  &  43           \\ %\hline
        \specialrule{.15em}{.0em}{0em} 
            \textbf{RMAPPO}           & \textbf{Global}          &   \textbf{173.13}     & \textbf{0.41}  &        \textbf{0.67}   &  \textbf{96} &     \textbf{327.39}   & \textbf{0.44}  &      \textbf{4.29}    &  \textbf{88}    &  \textbf{366.81}      &  \textbf{0.44} &   \textbf{6.93}  &  \textbf{79}        \\ \specialrule{.15em}{.0em}{0em} %\hline
        % GPG (static)      & Local       &   $-67.03$     &  $0.96$ &      $1.47$     &  7  &  $-180.14$      & $0.99$  &      $6.41$     &   1 &    -182.57    & 1.00  &   9.44   &    0     \\ \hline
        GPG (dyn.)    & Local       &   $-46.27$     &  $0.87$ &     $0.21$     &   8  &  $-165.91$       & $1.00$  &        $1.57$       &  3  & -173.53  &  1.00 &   2.24   &    0     \\ \hline
        % DGN               & Local       &    $32.94$    & $0.59$  &       $2.57$    &   32 &  $-232.32$      & $0.97$  &       $5.39$   &  0   &     -243.45   & 1.00  &   8.62  &     0     \\ \hline
        DGN+ATOC       & Local       &    $67.70$    &  $0.66$ &      $0.72$         &  35  &  $-189.61$  & $0.97$  &      $1.03$    &  0   &   -201.01     & 1.00  &   1.97   &  0       \\ \hline
        EMP              & Local       &  $-83.96$      &  $0.98$ &       $0.72$     & 6   &  $-211.90$      & $0.98$  &     $2.63$   &    0  & -209.90   & 1.00  &  94.12   &    0      \\ %\hline
        \specialrule{.15em}{.0em}{0em} 
   %     RMAPPO \cite{MAPPO}           & Global          &   $173.13$     & $0.41$  &        $1.47$   &  96 &     $327.39$   & $0.44$  &      $8.64$    &  88    &  366.81      &  0.44 &   13.21  &  79        \\ \hline
        \textbf{InforMARL} & \textbf{Local} &     \textbf{205.24}   & \textbf{0.17}  &       \textbf{1.45}    &  \textbf{100}  &     \textbf{399.01}   &  \textbf{0.37} &  \textbf{3.72}    &  \textbf{100}       &  \textbf{429.14}      &  \textbf{0.39} &  \textbf{4.73}   & \textbf{100}          \\ 
         \specialrule{.15em}{.0em}{0em} 
        %\hline
        \end{tabular}
        \setlength{\belowcaptionskip}{-12pt}
        \caption{Comparison of InforMARL with the best-performing baseline methods, for the \emph{Target} task environment with 3, 7, and 10 agents, averaged over 100 test episodes. See Appendix \ref{appendix:full_comparison} for comparisons to other baseline methods.
        % The following metrics are compared: (a) Total reward obtained in an episode by all the agents (higher is better). (b) Fraction of episode taken by the agents to reach the goal, \textbf{$T$} (lower is better). (c)   The total number of collisions the agents had in the episode, \# col (lower is better). (d) Percent of episodes in which all agents are able to get to their goals, $S$\% (higher is better). The best-performing methods that use global information (RMAPPO) and local information (InforMARL) are highlighted. As noted in Section \ref{sec:comparison_algos}, the metrics \# col and $S$ should be considered on balance.
        }
        \label{table:comparison}
        % Reward: Total reward obtained over the episode (higher the better). T: The average fraction of an episode taken by the all agent to reach their respective goals (lower the better).  No. of Collisions: The total number of collisions the agents had (agent-agent + agent-obstacle) in the episode (lower the better). Although, having a smaller number of collisions is better, some policies do not move at all and do not get to the goal and hence may have lesser collisions. So this metric should be compared with the success rate `S\%' in context. $\dagger$-the original implementation assumes that the positions of all the entities in the environment are known at the beginning of the episode}
    \end{table*}
    
    We present the following metrics in Table \ref{table:comparison}. The results represent an average over 100 test episodes.
    \begin{CompactEnumerate}
        \item The total rewards obtained by the agents during an episode 
        % using the reward function defined in Section \ref{section:env}. 
        A higher value corresponds to better performance.
        \item The fraction of an episode that the agents take on average to get to the goal, denoted $T$. If an agent does not reach its goal, then $T$ is set to be 1 (lower is better).
        \item Percent of episodes in which all agents are able to get to their goals, denoted $S$\% (higher is better).
        \item The total number of collisions (both agent-agent + agent-obstacle) that agents had in an episode, denoted \# col. The lower this metric, the better the performance of the algorithm. 
    \end{CompactEnumerate}
    Although having a smaller number of collisions is better, the policies of some of the baseline algorithms do not significantly move the agents from their initial position after training and hence do not get to the goal. This leads to them having a lower number of collisions. Hence, this metric should be judged with the success rate in context.
    % \textbf{Rewards}: The total rewards obtained by the agents during the episode using the reward function defined in \ref{section:env} (Higher is better). \textbf{T}: Fraction of episode the agents take to get to the goal. If they do not reach the goal then T is set to be 1. \textbf{Number of Collisions} (\# of col): The total number of collisions the agents had (agent-agent + agent-obstacle) in the episode (Lower is better). Although having a smaller number of collisions is better, the policies of some of the baseline algorithms do not move the agents much from their initial position after training and hence do not get to the goal. This leads to them having lesser number of collisions. Hence, this metric should be judged with the success-rate in context. \textbf{Success Rate} (S\%): In what percentage of episodes are all the agents able to get to their goals (Higher is better).\\
    
    The graph-based methods, namely GPG (static and dynamic), DGN (+ATOC), and EMP do not learn effectively with local information modes. Although both GPG and DGN use GCNs, they do not perform as well as InforMARL because they use only agent-agent and not agent-entity graphs. The lack of information about non-agent entities means that agents cannot maneuver through the environment to avoid collisions.
    % Both GPG and DGN are not able to learn optimal policies because the graphs they use do not have other entities in them which leads to them not getting any information about their positions. 
   
   In contrast to the results showed in \cite{GPG}, our results show that the dynamic graph version of GPG is slightly better than the static graph one. A possible reason for this discrepancy is that the fixed formation environment considered in \cite{GPG} is more amenable to the use of static graphs than the navigation environment. EMP, which uses a similar agent-entity graph as ours, fails to learn because of the strong assumption of having access to the positions of all entities in the environment at the beginning of the episode. The original implementation of EMP (and the associated environments) included information about all the entities other than agents in the observation vector.

   % \begin{table*}
   % \centering
   %      \begin{tabular}{|p{1.5cm}||p{1.9cm}||c||c|r|c||c|r|c||}
   %      \hline
   %      \multirow{2}{*}{Task} & \multirow{2}{*}{Algorithm} & Info & \multicolumn{3}{c||}{$m=3$} & \multicolumn{3}{c||}{$m=7$}\\
   %      \cline{4-9}
   %       & & mode & $T$ & \# col  & $S\%$  & $T$ & \# col & $S\%$\\
   %  \hline \hline
   %      Coverage & RMADDPG          & Global          &  $0.75$ &         $3.20$   &  23  & $0.95$  & $9.75$ &  3 \\ 
   %      \hline
   %      Coverage & RMATD3           & Global         & $0.51$  &     $3.07$      &  67   & $0.96$  &      $7.40$         &  6\\ 
   %      \hline
   %      Coverage & RQMIX           & Global            &  $0.77$ &       $1.42$     & 28     & $0.85$  &    $11.5$      & 12 \\ 
   %      \hline
   %      Coverage & RVDN             & Global          &  $0.62$ &          $1.05$     &  45  &    $0.62$ &       $6.60$   &   47  \\ %\hline
   %      \specialrule{.2em}{.0em}{0em} 
        
   %      Coverage & \textbf{RMAPPO}           & \textbf{Global}        & \textbf{0.41}  &        \textbf{1.47}   &  \textbf{96} &      \textbf{0.44}  &      \textbf{8.64}    &  \textbf{88}    \\ 
   %          \specialrule{.2em}{.0em}{0em} %\hline
   %      Coverage & GPG(dynamic)    & Local         &  $0.87$ &     $0.43$     &   8 & $1.00$  &        $3.20$       &  3  \\ 
   %      \hline
   %      Coverage & DGN+ATOC       & Local          &  $0.66$ &      $1.49$         &  35  & $0.97$  &      $2.20$    &  0       \\ 
   %      \hline
   %      Coverage & EMP              & Local         &  $0.98$ &       $1.35$     & 6   & $0.98$  &     $5.91$   &    0  \\ %\hline
   %      \specialrule{.2em}{.0em}{0em} 
   %      Coverage & \textbf{InforMARL} & \textbf{Local} &      \textbf{0.38}  &       \textbf{1.45}    &  \textbf{100}   &  \textbf{0.37} &  \textbf{6.97}    &  \textbf{100}\\ 
   %       \specialrule{.2em}{.0em}{0em} 
   %      %\hline
   %      \end{tabular}
   %      \caption{Comparison of InforMARL with other baseline methods, for scenarios with 3 agents in the coverage, formation and line environments. The results presented represent the average of 100 test episodes. The best-performing methods that use global information (RMAPPO) and local information (InforMARL) are highlighted. As noted in Section \ref{sec:comparison_algos}, the metrics \# col and $S$ should be considered on balance.
   %      }
   %      \label{table:comparison2}
   %  \end{table*}

% \begin{table*}[h]
%     \centering
%         \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
%         % \specialrule{.2em}{.0em}{0em} 
%         \hline
%         \multirow{2}{*}{Task}& \multirow{2}{*}{$m$} & \multirow{2}{*}{Metric} & \multicolumn{6}{c|}{Algorithm}\\ 
%         \cline{4-9}
%         & & & RMADDPG & RQMIX & RVDN & EMP$^\dagger$ & RMAPPO & InforMARL$^*$\\
%         % \specialrule{.2em}{.0em}{0em} 
%         \hline
%         \multirow{4}{*}{Coverage} & \multirow{2}{*}{3}& T & 0.41 & 0.39 & 0.38& & 0.34& 0.36 \\  \cline{3-9}
%         & & S\% & 93 & 95 & 96 & & 100 & 100         \\  \cline{2-9}
%         & \multirow{2}{*}{7}& T & 0.47 & 0.44 & 0.43 & &  0.42& 0.43 \\  \cline{3-8}
%         & & S\% & 92 & 94 & 95 & & 100 & 99         \\  \cline{1-9}

%         \multirow{4}{*}{Formation} & \multirow{2}{*}{3}& T & 1 & 2 & 3 & 4&& 5 \\  \cline{3-8}
%         & & S\% & 1 & 2 & 3 & &4& 5         \\  \cline{2-9}
%         & \multirow{2}{*}{7}& T & 1 & 2 & 3 && 4& 5 \\  \cline{3-9}
%         & & S\% & 1 & 2 & 3 & &4& 5         \\  \cline{1-9}

%         \multirow{4}{*}{Line} & \multirow{2}{*}{3}& T & 1 & &2 & 3 & 4& 5 \\  \cline{3-8}
%         & & S\% & 1 & 2 & &3 & 4& 5         \\  \cline{2-9}
%         & \multirow{2}{*}{7}& T & 1 && 2 & 3 & 4& 5 \\  \cline{3-9}
%         & & S\% & 1 & 2 & 3 & &4& 5         \\  \cline{1-9}
%         \end{tabular}
%         \caption{Only InforMARL was trained on the 3 agent scenario and tested on $m=\{3,7\}$ agents whereas all other algorithms were trained and tested on the corresponding number of agents.}
%         \label{table:transfer2}
%     \end{table*}

\subsection{Scalability of InforMARL}
    To evaluate the scalability of InforMARL with minimum information, we perform experiments in the \emph{Target} environment by testing the models in scenarios with a different number of agents from those they were trained on. 
%      \begin{table}[h]
%         \begin{tabular}{|l|c||c|c|c|}
%         % \specialrule{.2em}{.0em}{0em} 
%         \hline
%         \multicolumn{2}{|c||}{\diagbox{Test}{Train}}& $n=3$  & $n=7$ & $n=10$\\ 
%         % \specialrule{.2em}{.0em}{0em} 
%         \hline\hline
%             % \diagbox{Train}{Test}
%             % &\makebox[3em]{5/31}&\makebox[3em]{6/1}&\makebox[3em]{6/2}
%             % &\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
%             \multirow{4}{*}{$m=3$} 
%             & Reward/$m$ & 68.41 & 58.30 & 57.27\\ \cline{2-5}
%             & $T$ & 0.38 & 0.38 & 0.39\\ \cline{2-5}
%             & (\# col)/m & 0.48 & 0.61 & 0.64\\ \cline{2-5}
%             & $S\%$ & 100 & 100 & 99\\
% %            \specialrule{.2em}{.0em}{0em} 
%              \hline\hline
            
%             \multirow{4}{*}{$m=7$} 
%             & Reward/$m$ & 61.16 & 57.00 & 58.32\\ \cline{2-5}
%             & $T$ & 0.38 & 0.37 & 0.38\\ \cline{2-5}
%             & (\# col)/$m$ & 1.15 & 0.99 & 1.03\\ \cline{2-5}
%             & $S\%$ & 100 & 100 & 100\\
%  %           \specialrule{.2em}{.0em}{0em} 
%               \hline\hline
            
%             \multirow{4}{*}{$m=10$} 
%             & Reward/$m$ & 58.59 & 53.25 & 52.10\\ \cline{2-5}
%             & $T$ & 0.38 & 0.38 & 0.39\\ \cline{2-5}
%             & (\# col)/$m$ & 1.60 & 1.43 & 1.68\\ \cline{2-5}
%             & $S\%$ & 100 & 99 & 100\\ %\specialrule{.2em}{.0em}{0em} 
%             \hline \hline 
%             \multirow{4}{*}{$m=15$} 
%             & Reward/$m$ & 53.19 & 46.39 & 48.15\\ \cline{2-5}
%             & $T$ & 0.39 & 0.39 & 0.40\\ \cline{2-5}
%             & (\# col)/$m$ & 2.24 & 2.314 & 2.20\\ \cline{2-5}
%             & $S\%$ & 100 & 99 & 99\\
%             % \specialrule{.2em}{.0em}{0em} 
%             \hline
%         \end{tabular}
%         \caption{Test performance of InforMARL, when trained on scenarios with $n$ agents and tested on scenarios with $m$ agents in the environment. InforMARL is able to achieve a success rate of nearly 100\%  while the fraction of episodes taken to reach the goals ($T$) is almost constant. Note that we normalize the reward and the number of collisions by $m$ for ease of comparison.}
%         \label{table:transfer}
%     \end{table}

    \begin{table}[h]\small\centering
        \begin{tabular}{|l|c||c|c|c|}
        % \specialrule{.2em}{.0em}{0em} 
        \hline
        \multicolumn{2}{|c||}{\diagbox{\bf Test}{\bf Train}}& $\boldsymbol{n=3}$  & $\boldsymbol{n=7}$ & $\boldsymbol{n=10}$\\ 
        % \specialrule{.2em}{.0em}{0em} 
        \hline\hline
            % \diagbox{Train}{Test}
            % &\makebox[3em]{5/31}&\makebox[3em]{6/1}&\makebox[3em]{6/2}
            % &\makebox[3em]{6/3}&\makebox[3em]{6/4}\\\hline\hline
            \multirow{4}{*}{$\boldsymbol{m=3}$} 
            & Reward/$m$ & 63.21 & 63.25 & 62.87\\ \cline{2-5}
            & $T$ & 0.39 & 0.40 & 0.40\\ \cline{2-5}
            & (\# col)/m & 0.40 & 0.46 & 0.49\\ \cline{2-5}
            & $S\%$ & 100 & 100 & 99\\
%            \specialrule{.2em}{.0em}{0em} 
             \hline\hline
            
            \multirow{4}{*}{$\boldsymbol{m=7}$} 
            & Reward/$m$ & 61.16 & 62.23 & 61.32\\ \cline{2-5}
            & $T$ & 0.38 & 0.40 & 0.40\\ \cline{2-5}
            & (\# col)/$m$ & 0.74 & 0.66 & 0.70\\ \cline{2-5}
            & $S\%$ & 100 & 100 & 100\\
 %           \specialrule{.2em}{.0em}{0em} 
              \hline\hline
            
            \multirow{4}{*}{$\boldsymbol{m=10}$} 
            & Reward/$m$ & 58.59 & 58.23 & 58.67\\ \cline{2-5}
            & $T$ & 0.38 & 0.40 & 0.39\\ \cline{2-5}
            & (\# col)/$m$ & 0.95 & 0.88 & 0.87\\ \cline{2-5}
            & $S\%$ & 100 & 99 & 100\\ %\specialrule{.2em}{.0em}{0em} 
            \hline \hline 
            \multirow{4}{*}{$\boldsymbol{m=15}$} 
            & Reward/$m$ & 53.19 & 53.46 & 54.21\\ \cline{2-5}
            & $T$ & 0.39 & 0.40 & 0.40\\ \cline{2-5}
            & (\# col)/$m$ & 1.28 & 1.21 & 1.20\\ \cline{2-5}
            & $S\%$ & 100 & 99 & 99\\
            % \specialrule{.2em}{.0em}{0em} 
            \hline
        \end{tabular}
%        \setlength{\belowcaptionskip}{-14pt}
        \caption{Test performance of InforMARL for the \emph{Target} task, when trained on scenarios with $n$ agents and tested with $m$ agents in the environment.
        % InforMARL is able to achieve a success rate of nearly 100\%  while the fraction of episodes taken to reach the goals ($T$) is almost constant. 
        % Note that we normalize the reward and the number of collisions by $m$ for ease of comparison.
        }
        \label{table:transfer}
    \end{table}
    
    Table \ref{table:transfer} shows the results of testing InforMARL trained on $n$ agents and tested on $m$ agents. Each scenario is tested over 100 episodes. The number of obstacles in the environment is randomly chosen from $(0,10)$ at the beginning of the episode. Based on the findings presented in Table \ref{table:comparison}, we did not test the scalability of other methods since they did not perform well in the local information mode, or could not handle varying numbers of entities in the environment.  
    
    We see from  Table \ref{table:transfer} that InforMARL is able to achieve a success rate of 100\% for almost all the scenarios when the number of agents in the environment as varied. Furthermore, with InforMARL, the agents are able to get to their goals within $T \sim 0.39$ of the episode length in all scenarios. The number of collisions per agent increases, which is to be expected as the environment becomes denser. We believe that this can be remedied by using a stricter penalty %(negative reward) 
    for collisions. %instead of the $-5$ penalty used in our experiments. 
    Alternatively, %a more sophisticated approach with 
    control barrier functions for satisfying safety constraints could be used to provide a formal safety guarantee in the MARL setting \cite{MARL_control_barrier}.

\subsection{Performance in Other Task Environments\label{sec:other_tasks}}
% - These environments are more complex, in the sense that they require more coordination among agents.
In the \emph{Target} task environment, coordination amongst agents was required only for collision avoidance (both with other agents and obstacles) since the goal positions for all the agents were predetermined. For the \emph{Coverage}, \emph{Formation} and \emph{Line} tasks, the agents not only need to coordinate for collision avoidance but also need to develop  consensus on their goals. Table \ref{table:transfer2} shows the success rate and the fraction of episode taken to complete the task in the \emph{Coverage}, \emph{Formation} and \emph{Line} environments. Here, InforMARL was trained in the 3-agent scenario and tested on the 3- and 7-agent scenarios, whereas RMAPPO is trained and tested on scenarios with the same number of agents. InforMARL is able to achieve a success rate of almost 100\% across all scenarios in the different environments, while taking a similar fraction of the episode to complete as RMAPPO. While RMAPPO requires global information to learn a successful policy, InforMARL only needs local neighborhood information. This illustrates the effectiveness of the information aggregation module in InforMARL when the agents only have access to local information.
% In Target environment, coordination essentially was required for collision avoidance maneuvers (both with other agents as well as static obstacles), since the goal positions for all the agents were known in advance. In Coverage, Formation and Line environments, agents are not only required to coordinate for the purposes of collision avoidance, but also coordinate amongst themselves to determine their goal destination. This necessitates the requirement of global information even for the purposes of successfully completing the task, let alone perform them optimally. 

% Observation:
%     - success rate is still 100\%
%     - total travel time is smaller, or similar
% Significance:
%     - Informarl is Trained on just 3 agents and works as well as mappo which was trained on 7 agents.
%     - Informarl still uses local information whereas mappo uses global


% Thoughts:
% 1. In terms of environment complexity, formation = line > coverage > target
% 2. Explain why? Maybe in appendix


    \begin{table}[h]
    \small\centering
        \begin{tabular}{|c|c|c|c|c|}
        % \specialrule{.2em}{.0em}{0em} 
        \hline
        \multirow{2}{*}{\bf Environment}& \multirow{2}{*}{$\boldsymbol{m}$} & \multirow{2}{*}{\bf Metric} & \multicolumn{2}{c|}{\bf Algorithm}\\ 
        \cline{4-5}
        & & &  {\bf RMAPPO} & {\bf InforMARL}\\
        % \specialrule{.2em}{.0em}{0em} 
        \hline\hline
        \multirow{4}{*}{\bf Coverage} & \multirow{2}{*}{3}& $T$ &  0.34& 0.36 
        \\  \cline{3-5}
        & & $S\%$ &  100 & 100
        \\  \cline{2-5}
        & \multirow{2}{*}{7}& $T$ &   0.42& 0.43 
        \\  \cline{3-5}
        & & $S\%$ &  100 & 99
        \\   \specialrule{.12em}{.0em}{0em}
        \multirow{4}{*}{\bf Formation} & \multirow{2}{*}{3}& $T$ & 0.31 & 0.30 
        \\  \cline{3-5}
        & & $S\%$ & 100 & 100
        \\  \cline{2-5}
        & \multirow{2}{*}{7}& $T$ &  0.47& 0.43
        \\  \cline{3-5}
        & & $S\%$ & 100& 100
        \\   \specialrule{.12em}{.0em}{0em}
        \multirow{4}{*}{\bf Line} & \multirow{2}{*}{3}& $T$ &  0.24& 0.21 \\  
        \cline{3-5}
        & & $S\%$ &  100 & 100
        \\  \cline{2-5}
        & \multirow{2}{*}{7}& $T$ & 0.38& 0.36  \\
        \cline{3-5}
        & & $S\%$ & 100 & 100
        \\  \hline
        \end{tabular}
         \setlength{\belowcaptionskip}{-8pt}
        \caption{Performance of RMAPPO and InforMARL on the \emph{coverage}, \emph{formation}, and \emph{line} tasks. We note that InforMARL was trained on the 3-agent scenario and tested on $m=\{3,7\}$ agents, while RMAPPO was trained and tested on the same number of agents (\ie with $m=n$). %RMAPPO uses global information whereas InforMARL just uses local information.
        }
        \label{table:transfer2}
    \end{table}
   



==> icml2023 InforMARL 2/sections/5_conclusion_future.tex <==
\section{Conclusions and Future Work}
\label{section:conclusion_future_work}
We introduced InforMARL, a novel architecture that uses GNNs for scalable multi-agent reinforcement learning. We showed that having just local observations as states is not enough for standard MARL algorithms to learn meaningful policies. Along with this, we also showed that albeit na{\"i}vely concatenating state information about all the entities in the environment helps to learn good policies, they are not transferable to other scenarios with a different number of entities than what it was trained on. InforMARL is able to learn transferable policies using standard MARL algorithms using just local observations and an aggregated neighborhood information vector. Furthermore, it has better sample complexity than other standard MARL algorithms that use global observation. We demonstrated these findings for four environments with different navigation tasks: \emph{target}, \emph{coverage}, \emph{formation}, and \emph{line}.  
Future work will include the introduction of more complex (potentially adversarial) dynamic obstacles in the environment and adding a safety guarantee layer for the actions of the agents to avoid collisions. Additionally, the use of InforMARL for curriculum learning and transfer learning to different environments %\cite{transfer_learning1, transfer_learning2, curriculum_learning} 
is a topic of ongoing research. 
% Future work includes having more complex dynamic obstacles (adversarial) in the environment and adding a safety guarantee layer for the actions of the agents to avoid collisions at all costs. Since the usage of graph information aggregation allows for transferring learning to different scenarios, investigating curriculum learning \cite{transfer_learning1, transfer_learning2, curriculum_learning} to test out the effectiveness of InforMARL with learning in an environment different than the ones it was trained on.

==> icml2023 InforMARL 2/sections/6_acknowledgement.tex <==
% Acknowledge Supercloud for their awesome system and NASA/USAF for money$$$$$
\section*{Acknowledgements}
The authors would like to thank the MIT SuperCloud
\cite{supercloud} and the Lincoln Laboratory Supercomputing Center for providing high performance computing resources that have contributed to the research results reported
within this paper. The NASA University Leadership initiative (grant \#80NSSC20M0163) provided funds to assist the authors with their research, but this article solely reflects the opinions and conclusions of its authors and not any NASA entity. This research was sponsored in part by the United States AFRL and the United States Air Force Artificial Intelligence Accelerator and was accomplished under Cooperative Agreement Number FA8750-19-2-1000. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the United States Air Force or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notion herein.

